Static Energy in ($2+1+1$)-Flavor Lattice QCD: Scale Setting and Charm Effects

We present results for the static energy in ($2+1+1$)-flavor QCD over a wide range of lattice spacings and several quark masses, including the physical quark mass, with ensembles of lattice-gauge-field configurations made available by the MILC Collaboration. We obtain results for the static energy out to distances of nearly $1$~fm, allowing us to perform a simultaneous determination of the scales $r_{1}$ and $r_{0}$, as well as the string tension $\sigma$. For the smallest three lattice spacings we also determine the scale $r_{2}$. Our results for $r_{0}/r_{1}$ and $r_{0}\sqrt{\sigma}$ agree with published ($2+1$)-flavor results. However, our result for $r_{1}/r_{2}$ differs significantly from the value obtained in the ($2+1$)-flavor case, which is most likely due to the effect of the charm quark. We also report results for $r_{0}$, $r_{1}$, and $r_{2}$ in~fm, with the former two being slightly lower than published ($2+1$)-flavor results. We study in detail the effect of the charm quark on the static energy by comparing our results on the finest two lattices with the previously published ($2+1$)-flavor QCD results at similar lattice spacing. We find that for $r > 0.2$~fm our results on the static energy agree with the ($2+1$)-flavor result, implying the decoupling of the charm quark for these distances. For smaller distances, on the other hand, we find that the effect of the dynamical charm quark is noticeable. The lattice results agree well with the two-loop perturbative expression of the static energy incorporating finite charm mass effects. This is the first time that the decoupling of the charm quark is observed and quantitatively analyzed on lattice data of the static energy.

==> paper_scales_tables/fit_intervals.tex <==
$\approx a$~(fm)& $\beta$ & $\sfrac{\tmax}{a}$ & \tmax~(fm) & Operator & $\sfrac{r_{I}}{a}$
& $\sfrac{\tmin^{(1,-)}}{a}$ & $\sfrac{\tmin^{(2,-)}}{a}$ & $\sfrac{\tmin^{(3,-)}}{a}$
& $\sfrac{\tmin^{(1,0)}}{a}$ & $\sfrac{\tmin^{(2,0)}}{a}$ & $\sfrac{\tmin^{(3,0)}}{a}$
& $\sfrac{\tmin^{(1,+)}}{a}$ & $\sfrac{\tmin^{(2,+)}}{a}$ & $\sfrac{\tmin^{(3,+)}}{a}$ \\
\hline
\mrow{3}{0.15\h} &  \mrow{3}{5.8\h}  &   \mrow{3}{9} &  \mrow{3}{1.35}
&  Bare             &  all
&     1             &     1             &   --
&     2             &     2             &   --
&     3             &     3             &   --     \\
\cline{5-15}
&                   &                   &
&  \mrow{2}{Hyp}    &  \phantom{0.0}--3.5
&     1             &     1             &   2
&     2             &     2             &   2
&     3             &     3             &   2      \\
&                   &                   &
&                   &  3.5--\phantom{0.0}
&     1             &     1             &   1
&     2             &     2             &   1
&     3             &     3             &   1      \\
\hline
\hline
\mrow{4}{0.12\h} &  \mrow{4}{6.0\h}  &   \mrow{4}{6} &  \mrow{4}{0.73}
&  \mrow{2}{Bare}   &  \phantom{0.0}--1.6
&     2             &     2             &   --
&     3             &     2             &   --
&     --            &     --            &   --     \\
&                   &                   &
&                   &  1.6--\phantom{0.0}
&     2             &     2             &   --
&     3             &     2             &   --
&     --            &     --            &   --     \\
\cline{5-15}
&                   &                   &
&  \mrow{2}{Hyp}    &   \phantom{0.0}--3.5
&     2             &     2             &   1
&     3             &     2             &   1
&     --            &     --            &   --     \\
&                   &                   &
&                   &  3.5--\phantom{0.0}
&     2             &     2             &   --
&     3             &     2             &   1
&     --            &     --            &   --     \\
\hline
\hline
\mrow{5}{0.088}  &   \mrow{5}{6.3\h} &   \mrow{5}{8} &  \mrow{5}{0.70}
&  \mrow{3}{Bare}   &   \phantom{0.0}--1.0
&     3             &     1             &   2
&     4             &     2             &   2
&     5             &     3             &   2      \\
&                   &                   &
&                   &   1.0--3.5
&     3             &     2             &   2
&     4             &     3             &   2
&     5             &     3             &   2      \\
&                   &                   &
&                   &   3.5--\phantom{0.0}
&     3             &     2             &   1
&     4             &     3             &   1
&     5             &     3             &   1      \\
\cline{5-15}
&                   &                   &
&  \mrow{2}{Hyp}    &   \phantom{0.0}--3.5
&     3             &     3             &   2
&     4             &     3             &   2
&     5             &     3             &   2      \\
&                   &                   &
&                   &   3.5--\phantom{0.0}
&     3             &     3             &   1
&     4             &     3             &   1
&     5             &     3             &   1      \\
\hline
\hline
\mrow{10}{0.057} &   \mrow{10}{6.72} &   \mrow{10}{10} &  \mrow{10}{0.57}
&  \mrow{5}{Bare}   &   \phantom{0.0}--1.6
&     4             &     3             &   2
&     5             &     3             &   2
&     6             &     4             &   2      \\
&                   &                   &
&                   &   1.6--1.9
&     5             &     3             &   2
&     6             &     4             &   2
&     7             &     4             &   2      \\
&                   &                   &
&                   &   1.9--3.0
&     5             &     3             &   2
&     6             &     4             &   2
&     7             &     5             &   2      \\
&                   &                   &
&                   &   3.0--3.5
&     5             &     3             &   2
&     6             &     4             &   2
&     7             &     5             &   3      \\
&                   &                   &
&                   &   3.5--\phantom{0.0}
&     5             &     3             &   1
&     6             &     4             &   2
&     7             &     5             &   3      \\
\cline{5-15}
&                   &                   &
&  \mrow{5}{Hyp}    &   \phantom{0.0}--1.6
&     4             &     3             &   2
&     5             &     3             &   2
&     6             &     4             &   2      \\
&                   &                   &
&                   &   1.6--1.9
&     5             &     3             &   2
&     6             &     3             &   2
&     7             &     4             &   2      \\
&                   &                   &
&                   &   1.9--3.0
&     5             &     3             &   2
&     6             &     4             &   2
&     7             &     5             &   2      \\
&                   &                   &
&                   &   3.0--3.5
&     5             &     3             &   2
&     6             &     4             &   2
&     7             &     5             &   3      \\
&                   &                   &
&                   &   3.5--\phantom{0.0}
&     5             &     3             &   1
&     6             &     4             &   2
&     7             &     5             &   3      \\
\hline
\hline
\mrow{16}{0.042} &  \mrow{16}{7.0\h} &  \mrow{16}{20} &  \mrow{16}{0.85}
&  \mrow{9}{Bare}   &   \phantom{0.0}--1.0
&     5             &     3             &   2
&     6             &     3             &   2
&     7             &     4             &   2      \\
&                   &                   &
&                   &   1.0--2.4
&     6             &     3             &   2
&     7             &     4             &   2
&     8             &     5             &   2      \\
&                   &                   &
&                   &   2.4--2.7
&     6             &     3             &   2
&     8             &     4             &   2
&     9             &     5             &   2      \\
&                   &                   &
&                   &   2.7--3.0
&     7             &     4             &   2
&     8             &     5             &   2
&     9             &     6             &   2      \\
&                   &                   &
&                   &   3.0--3.5
&     7             &     4             &   2
&     8             &     5             &   2
&     9             &     6             &   3      \\
&                   &                   &
&                   &   3.5--3.8
&     7             &     4             &   1
&     8             &     5             &   2
&     9             &     6             &   3      \\
&                   &                   &
&                   &   3.8--6.0
&     7             &     5             &   1
&     8             &     6             &   2
&     9             &     7             &   3      \\
&                   &                   &
&                   &   6.0--9.0
&     7             &     5             &   2
&     8             &     6             &   3
&     9             &     7             &   4      \\
&                   &                   &
&                   &   9.0--\phantom{0.0}
&     7             &     5             &   3
&     8             &     6             &   4
&     9             &     7             &   5      \\
\cline{5-15}
&                   &                   &
&  \mrow{7}{Hyp}    &   \phantom{0.0}--2.5
&     6             &     3             &   2
&     8             &     4             &   2
&     7             &     4             &   2      \\
&                   &                   &
&                   &   2.5--3.0
&     7             &     4             &   2
&     8             &     5             &   2
&     8             &     5             &   2      \\
&                   &                   &
&                   &   3.0--3.5
&     7             &     4             &   2
&     8             &     5             &   2
&     8             &     5             &   2      \\
&                   &                   &
&                   &   3.5--3.8
&     7             &     4             &   1
&     8             &     5             &   1
&     8             &     5             &   2      \\
&                   &                   &
&                   &   3.8--6.0
&     7             &     5             &   1
&     8             &     6             &   1
&     8             &     6             &   2      \\
&                   &                   &
&                   &   6.0--9.0
&     7             &     5             &   2
&     8             &     6             &   2
&     8             &     6             &   3      \\
&                   &                   &
&                   &   9.0--\phantom{0.0}
&     7             &     5             &   3
&     8             &     6             &   3
&     8             &     6             &   4      \\
\hline
\hline
\mrow{27}{0.032} &   \mrow{27}{7.28} &  \mrow{27}{28} &  \mrow{27}{0.91}
&  \mrow{14}{Bare}  &   \phantom{0.0}--1.0
&     7             &     3             &   2
&     8             &     4             &   2
&     9             &     5             &   2      \\
&                   &                   &
&                   &   1.0--1.6
&     7             &     4             &   2
&     8             &     5             &   2
&     9             &     6             &   2      \\
&                   &                   &
&                   &   1.6--2.5
&     8             &     4             &   2
&     9             &     5             &   2
&     10            &     6             &   2      \\
&                   &                   &
&                   &   2.5--2.8
&     9             &     4             &   2
&     9             &     5             &   2
&     10            &     6             &   2      \\
&                   &                   &
&                   &   2.8--2.9
&     9             &     4             &   2
&     10            &     5             &   2
&     11            &     6             &   2      \\
&                   &                   &
&                   &   2.9--3.0
&     9             &     5             &   2
&     10            &     6             &   2
&     11            &     7             &   2      \\
&                   &                   &
&                   &   3.0--3.5
&     9             &     5             &   2
&     10            &     6             &   2
&     11            &     7             &   3      \\
&                   &                   &
&                   &   3.5--4.3
&     9             &     5             &   1
&     10            &     6             &   2
&     11            &     7             &   3      \\
&                   &                   &
&                   &   4.3--5.8
&     9             &     6             &   1
&     10            &     7             &   2
&     11            &     8             &   3      \\
&                   &                   &
&                   &   5.8--6.0
&     9             &     7             &   1
&     10            &     8             &   2
&     11            &     9             &   3      \\
&                   &                   &
&                   &   6.0--9.0
&     9             &     7             &   2
&     10            &     8             &   3
&     11            &     9             &   4      \\
&                   &                   &
&                   &   9.0--12.0
&     9             &     7             &   3
&     10            &     8             &   4
&     11            &     9             &   5      \\
&                   &                   &
&                   &   12.0--15
&     9             &     7             &   4
&     10            &     8             &   5
&     11            &     9             &   6      \\
&                   &                   &
&                   &   15.0--\phantom{0.0}
&     9             &     7             &   5
&     10            &     8             &   6
&     11            &     9             &   7      \\
\cline{5-15}
&                   &                   &
&  \mrow{13}{Hyp}   &   \phantom{0.0}--1.7
&     7             &     4             &   2
&     8             &     5             &   2
&     9             &     6             &   2      \\
&                   &                   &
&                   &   1.7--2.5
&     8             &     4             &   2
&     9             &     5             &   2
&     10            &     6             &   2      \\
&                   &                   &
&                   &   2.5--2.8
&     9             &     4             &   2
&     9             &     5             &   2
&     11            &     6             &   2      \\
&                   &                   &
&                   &   2.8--2.9
&     9             &     4             &   2
&     10            &     5             &   2
&     11            &     6             &   2      \\
&                   &                   &
&                   &   2.9--3.0
&     9             &     5             &   2
&     10            &     6             &   2
&     11            &     7             &   2      \\
&                   &                   &
&                   &   3.0--3.5
&     9             &     5             &   2
&     10            &     6             &   2
&     11            &     7             &   3      \\
&                   &                   &
&                   &   3.5--4.3
&     9             &     5             &   1
&     10            &     6             &   2
&     11            &     7             &   3      \\
&                   &                   &
&                   &   4.3--5.8
&     9             &     6             &   1
&     10            &     7             &   2
&     11            &     8             &   3      \\
&                   &                   &
&                   &   5.8--6.0
&     9             &     7             &   1
&     10            &     8             &   2
&     11            &     9             &   3      \\
&                   &                   &
&                   &   6.0--9.0
&     9             &     7             &   2
&     10            &     8             &   3
&     11            &     9             &   4      \\
&                   &                   &
&                   &   9.0--12.
&     9             &     7             &   3
&     10            &     8             &   4
&     11            &     9             &   5      \\
&                   &                   &
&                   &   12.--15.
&     9             &     7             &   4
&     10            &     8             &   5
&     11            &     9             &   6      \\
&                   &                   &
&                   &   15.--\phantom{0.0}
&     9             &     7             &   5
&     10            &     8             &   6
&     11            &     9             &   7      \\


==> paper_scales_tables/only_LO_hyp_tree_avg.tex <==
\hline\hline
$\sfrac{x_{1}}{a}$ & $\sfrac{x_{2}}{a}$ & $\sfrac{x_{3}}{a}$ & Euclidean distance $\sfrac{|\bm{r}|}{a}$ &
Tree-level improved distance $\sfrac{r_{I}}{a}$ \\
\hline
% \hline ony one line in PRD style
1 & 0 & 0 & 1.0        & 1.4090720077683632 $\pm$ 0.0000272231574554 \\
1 & 1 & 0 & 1.41421356 & 1.6347902336183247 $\pm$ 0.0000465946237703 \\
1 & 1 & 1 & 1.73205081 & 1.8467595499778624 $\pm$ 0.0000720965811284 \\
2 & 0 & 0 & 2.0        & 2.0869639888379297 $\pm$ 0.00010881572881197901 \\
2 & 1 & 0 & 2.23606798 & 2.2824113277559475 $\pm$ 0.00014931241623131292 \\
2 & 1 & 1 & 2.44948974 & 2.46925261451723 $\pm$ 0.0001971166269616117 \\
2 & 2 & 0 & 2.82842712 & 2.8325399156211275 $\pm$ 0.0003189690177103989 \\
2 & 2 & 1 & 3.0 & 2.9968958678222193 $\pm$ 0.0003895871308315151 \\
3 & 0 & 0 & 3.0 & 3.019798092904878 $\pm$ 0.00040089572011213834 \\
3 & 1 & 0 & 3.16227766 & 3.1741224538042383 $\pm$ 0.0004792179268790236 \\
3 & 1 & 1 & 3.31662479 & 3.3230758478592826 $\pm$ 0.0005648652453895424 \\
2 & 2 & 2 & 3.46410162 & 3.4576827129777348 $\pm$ 0.0006490115003112156 \\
3 & 2 & 0 & 3.60555128 & 3.608266452442793 $\pm$ 0.0007606741720265368 \\
3 & 2 & 1 & 3.74165739 & 3.742820609162464 $\pm$ 0.0008680988507604019 \\
4 & 0 & 0 & 4.0 & 4.009312155119674 $\pm$ 0.001139908697499553 \\
3 & 2 & 2 & 4.12310563 & 4.123892762060447 $\pm$ 0.0012355323262901563 \\
4 & 1 & 0 & 4.12310563 & 4.1305992614166085 $\pm$ 0.0012695391549865612 \\
3 & 3 & 0 & 4.24264069 & 4.245403719802216 $\pm$ 0.001382495778147352 \\
4 & 1 & 1 & 4.24264069 & 4.248958125345892 $\pm$ 0.0014061580251402788 \\
3 & 3 & 1 & 4.35889894 & 4.361677691290871 $\pm$ 0.0015252521216272798 \\
4 & 2 & 0 & 4.47213595 & 4.477482540175397 $\pm$ 0.001702898505891101 \\
4 & 2 & 1 & 4.58257569 & 4.587800861080743 $\pm$ 0.0018601670608671774 \\
3 & 3 & 2 & 4.69041576 & 4.6943919313636595 $\pm$ 0.0019972646352736986 \\
4 & 2 & 2 & 4.89897949 & 4.904903016577305 $\pm$ 0.002375405660173766 \\
4 & 3 & 0 & 5.0 & 5.006341957150803 $\pm$ 0.0025732723487420857 \\
5 & 0 & 0 & 5.0 & 5.010612395918627 $\pm$ 0.0026663443713870827 \\
4 & 3 & 1 & 5.09901951 & 5.105848598131917 $\pm$ 0.0027642534122933175 \\
5 & 1 & 0 & 5.09901951 & 5.109317762292116 $\pm$ 0.002859977796668558 \\
3 & 3 & 3 & 5.19615242 & 5.2032779716044395 $\pm$ 0.002930317457110464 \\
5 & 1 & 1 & 5.19615242 & 5.206360898205104 $\pm$ 0.0030601624220681248 \\
4 & 3 & 2 & 5.38516481 & 5.393750119848208 $\pm$ 0.0033797564456950484 \\
5 & 2 & 0 & 5.38516481 & 5.395593701883427 $\pm$ 0.0034837603632714965 \\
5 & 2 & 1 & 5.47722558 & 5.487994029112106 $\pm$ 0.0037033882863966023 \\
4 & 4 & 0 & 5.65685425 & 5.6672919169514016 $\pm$ 0.004106445589974711 \\
4 & 4 & 1 & 5.74456265 & 5.755734149465888 $\pm$ 0.004343617910403466 \\
5 & 2 & 2 & 5.74456265 & 5.75676467951012 $\pm$ 0.004404424771737086 \\
4 & 3 & 3 & 5.83095189 & 5.842952338388262 $\pm$ 0.0045488594386881446 \\
5 & 3 & 0 & 5.83095189 & 5.843586389834391 $\pm$ 0.004667242236504972 \\
5 & 3 & 1 & 5.91607978 & 5.929386422609893 $\pm$ 0.004918742478458615 \\
4 & 4 & 2 & 6.0 & 6.013449483087768 $\pm$ 0.00509676734234446 \\
6 & 0 & 0 & 6.0 & 6.0172235033329935 $\pm$ 0.005440953835098437 \\
\hline\hline

==> paper_scales_tables/only_LO_tree_avg.tex <==
\hline\hline
$\sfrac{x_{1}}{a}$ & $\sfrac{x_{2}}{a}$ & $\sfrac{x_{3}}{a}$ & Euclidean distance $\sfrac{|\bm{r}|}{a}$ &
Tree-level improved distance $\sfrac{r_{I}}{a}$ \\
\hline
% \hline ony one line in PRD style
1 & 0 & 0 & 1.0 & 0.9599040344932587 $\pm$ 0.0000030136862000 \\
1 & 1 & 0 & 1.41421356 & 1.4333833568268333 $\pm$ 0.0000133976155673 \\
1 & 1 & 1 & 1.73205081 & 1.7866483317216775 $\pm$ 0.0000311330816800 \\
2 & 0 & 0 & 2.0 & 1.940263631933783 $\pm$ 0.0000494540199248 \\
2 & 1 & 0 & 2.23606798 & 2.2250232379448707 $\pm$ 0.0000808745459235 \\
2 & 1 & 1 & 2.44948974 & 2.4653405163348023 $\pm$ 0.00011862276324346516 \\
2 & 2 & 0 & 2.82842712 & 2.827620519955476 $\pm$ 0.0002078671683651496 \\
2 & 2 & 1 & 3.0 & 3.0128221441001566 $\pm$ 0.0002644187089284717 \\
3 & 0 & 0 & 3.0 & 2.9793711387856914 $\pm$ 0.0002645639904780199 \\
3 & 1 & 0 & 3.16227766 & 3.1516606507282003 $\pm$ 0.00032698001400311794 \\
3 & 1 & 1 & 3.31662479 & 3.315550137006213 $\pm$ 0.00039592619776753114 \\
2 & 2 & 2 & 3.46410162 & 3.477833619552443 $\pm$ 0.00046682948761451895 \\
3 & 2 & 0 & 3.60555128 & 3.6042808752983597 $\pm$ 0.0005498705705432746 \\
3 & 2 & 1 & 3.74165739 & 3.7462341283227087 $\pm$ 0.0006368426327038271 \\
4 & 0 & 0 & 4.0 & 3.9942805937128854 $\pm$ 0.0008554279175925462 \\
3 & 2 & 2 & 4.12310563 & 4.131365815324897 $\pm$ 0.0009318323950905256 \\
4 & 1 & 0 & 4.12310563 & 4.118890988277766 $\pm$ 0.000960436125197412 \\
3 & 3 & 0 & 4.24264069 & 4.244320104424595 $\pm$ 0.001049025250260445 \\
4 & 1 & 1 & 4.24264069 & 4.240985435735302 $\pm$ 0.0010718054244947838 \\
3 & 3 & 1 & 4.35889894 & 4.36364962603519 $\pm$ 0.0011653922807703446 \\
4 & 2 & 0 & 4.47213595 & 4.472231104277967 $\pm$ 0.0013133143767512239 \\
4 & 2 & 1 & 4.58257569 & 4.584957041812635 $\pm$ 0.0014420226596295169 \\
3 & 3 & 2 & 4.69041576 & 4.6983461132234074 $\pm$ 0.0015491618019277853 \\
4 & 2 & 2 & 4.89897949 & 4.904614883744731 $\pm$ 0.00186341000038508 \\
4 & 3 & 0 & 5.0 & 5.0034693599972435 $\pm$ 0.0020271029165576555 \\
5 & 0 & 0 & 5.0 & 5.000618027841458 $\pm$ 0.002126979684993836 \\
4 & 3 & 1 & 5.09901951 & 5.104096319382636 $\pm$ 0.0021838820081852054 \\
5 & 1 & 0 & 5.09901951 & 5.100261956285284 $\pm$ 0.0022864499838913307 \\
3 & 3 & 3 & 5.19615242 & 5.2052015467837895 $\pm$ 0.0023127731779240424 \\
5 & 1 & 1 & 5.19615242 & 5.198343994930819 $\pm$ 0.0024515745758860166 \\
4 & 3 & 2 & 5.38516481 & 5.392953837663012 $\pm$ 0.0026892417726260666 \\
5 & 2 & 0 & 5.38516481 & 5.3887915648408775 $\pm$ 0.00280178575059593 \\
5 & 2 & 1 & 5.47722558 & 5.481937186021168 $\pm$ 0.002983079856705198 \\
4 & 4 & 0 & 5.65685425 & 5.66330706933815 $\pm$ 0.003299445823816657 \\
4 & 4 & 1 & 5.74456265 & 5.752136910707054 $\pm$ 0.003494688720816784 \\
5 & 2 & 2 & 5.74456265 & 5.751750207016238 $\pm$ 0.0035622649763567037 \\
4 & 3 & 3 & 5.83095189 & 5.841093499561072 $\pm$ 0.0036533862067823692 \\
5 & 3 & 0 & 5.83095189 & 5.83774774213969 $\pm$ 0.0037834087253438733 \\
5 & 3 & 1 & 5.91607978 & 5.923873674850918 $\pm$ 0.003990944007350587 \\
4 & 4 & 2 & 6.0 & 6.009985877894033 $\pm$ 0.004115205044240455 \\
6 & 0 & 0 & 6.0 & 6.006755631439167 $\pm$ 0.004501425080677167 \\
\hline\hline
